Investigating an Intelligent System to Monitor \& Explain Abnormal Activity Patterns of Older Adults

Despite the growing potential of older adult care technologies, the adoption of these technologies remains challenging. In this work, we conducted a focus-group session with family caregivers to scope designs of the older adult care technology. We then developed a high-fidelity prototype and conducted its qualitative study with professional caregivers and older adults to understand their perspectives on the system functionalities. This system monitors abnormal activity patterns of older adults using wireless motion sensors and machine learning models and supports interactive dialogue responses to explain abnormal activity patterns of older adults to caregivers and allow older adults proactively sharing their status with caregivers for an adequate intervention. Both older adults and professional caregivers appreciated that our system can provide a faster, personalized service while proactively controlling what information is to be shared through interactive dialogue responses. We further discuss other considerations to realize older adult technology in practice.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.76.  Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.77.  Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.78.  Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.
	       

==> contents/design-opps-old.tex <==
\section{Design Opportunities and Recommendations}\label{sect:finding-designs}
Our qualitative evaluation details potential opportunities and limitations of the intelligent system that detects and explains an abnormal event of an older adult. Based on our findings and design activities with caregivers and older adults, we describe design opportunities and recommendations of the intelligent system for older adult care: additional use cases and functionalities and ways to support more trustful user engagement (Table \ref{tab:finding-designs}).


% Please add the following required packages to your document preamble:
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table}[h]
\centering
\caption{Summarized findings on design opportunities and recommendations of an intelligent system that detects and explains an abnormal event of an older adults}
\label{tab:finding-designs}
\resizebox{\textwidth}{!}{%
\begin{tabular}{cl}\toprule
\multirow{6}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Additional \\ Use Cases and Functionalities\end{tabular}}} &
  \begin{tabular}[c]{@{}l@{}}1. Monitoring other fine-level daily activities\\
  $\;\;\;$- Medication adherence\\$\;\;\;$- Attempt of standing up from a bed or a chair\\$\;\;\;$- Time to turn around for bedridden people\end{tabular} \\
   &
  2. Environmental monitoring: presence of others \& temperature \\
 &
  3. Physical assistance on transfer or feeding \\
 &
  4. Cognitive assistance \\

 &
  5. Validations on medical symptoms \\
 &
  6. Facilitate communications among professional \& family caregivers and doctors \\ \midrule
\multirow{5}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Ways for \\ Trustful User Engagement\end{tabular}}} &
  1. Tutorials \\
 &
  2. Multimodal sensing \& interactions \\
 &
  3. Explainable interactions \\
 &
  4. Personalized and privacy-aware interactions \\
 &
  5. Simple and intuitive designs \\ \bottomrule
\end{tabular}%
}
\end{table}

\subsection{Additional use cases \& functionalities}\label{sect:finding-designs-usecases}

\subsubsection{Monitoring other fine-level daily activities}


\begin{enumerate}
    \item Medication adherence
\end{enumerate}

%\subsubsection{}
%\hfill
%
%\noindent
All caregiver 

\textit{``Sometimes, we forget and past hours to take medications''} (O2), and \textit{``sometimes, I could not recall well whether I took my medicine or not''} (O5). \textit{``My father used to forget that he had taken his medicine so he would take it again''} (O1).
\textit{``Other possibilities, maybe medication takes (…) scheduled takings for certain times and alerts to not forget (…) especially antibiotics with schedule times''} (C1). \textit{``maybe it would be good to alert but you wouldn't be able to verify if they actually take it. Especially one with dementia (…) they pretend to take it (…) end up not taking it''} (C5). 

    

\subsubsection{Attempt of standing up}
\hfill

\noindent
\textit{``Even though some older adults know that they can’t get up by themselves, they are more more agitated or try to get up by themselves without ringing the bell. It would be useful to have a system to alert this event to avoid any dangerous situation (e.g. fall)''} (C5)
    

\subsubsection{Time to turn around bedridden people}
\hfill

\noindent
\textit{``Older adults who are bedridden should be turn around often, so as not to form wounds. However, it’s difficult to keep tracking the time to turn around each person. It would be useful to have an alert when it’s time to turn the bedridden people''} (C5).
    
\subsubsection{Physical assistance on transfer or feeding}
\hfill

\noindent
\textit{``Some older adults cannot drink or eat themselves. Especially, it would be good to alert the employee to give them water''} (C5). 
\textit{``If technologies would support to transfer an older adult from a bed to a wheelchair to an armchair would be very useful''} (C3). \textit{``This isn’t always possible alone as some older adults are very heavy''} (C4).
\textit{``In addition to monitoring the abnormal status, it would be useful to have a system that assists people who are no longer independent or do not have great motor skills''} (O3).
\textit{``For instance, my brother has Parkinson disease. He could not even get up by himself and need someone to help him. It would be good to have a system that can help him get up''} (O2)
    

\subsubsection{Cognitive Assistance}
\hfill

\noindent
\textit{``Now, I start forgetting most things''} (O3) \textit{``as I might forget about an important appointment (e.g. monthly hospital checkup), providing a reminder about an important event would be helpful too''} (O5).


\subsubsection{Environmental Monitoring: Presence of Others \& Temperature}
\hfill

\noindent
\textit{``detecting whether there is a new visitor in the house of an older adult would be useful to measure the level of socialization. Also, it would be good if the system can function to detect a dangerous invasion (e.g. thief) as surveillance for an older adult, who lives alone''} (O4).
\textit{``The medicine for my father, who had cancer, was very strong and he would be out of his mind. Once he almost set fire to his room, we got there in time, fortunately. Otherwise, he would have burned to death. Such monitoring would be very difficult when people live alone. It would be helpful if the system can also monitor the environmental abnormality (e.g. fire)''} (O1).
  
    
    
\subsubsection{Validations on medical symptoms}
\hfill

\noindent
\textit{``The example you gave of the bathroom. urinary infections are usually more common among women. in that case it would not be so important a food problem but a urinary infection''} (C5)
\textit{``If there is an emergency situation of an older adult, I wonder if the system can check up the older adult about the situation and medical symptoms''} (O4)

    

\subsubsection{Communications among professional \& family caregivers and doctors}
\hfill

\noindent  
\textit{``if some situation happens to an older adult, a family would need to make some decisions on behalf of an older adult. It would be better to have a communication channel between a health professional and a family member to determine a necessary intervention on behalf of an older adult''} (O5)
\textit{``If a system can share the status of an older adult and receive a remote medical appointment, that would be very helpful. One time, my mother-in-law had some rashes on her body, which were found while washing her. As my mother-in-law could not walk to the hospital, I asked for a visiting doctor and waited a few hours to receive a medical diagnosis. It would be great if the system can share the symptom of an older adult by videos instead of waiting for the visiting doctor''} (O4)

    
    


\subsection{Ways for Trustful User Engagement}\label{sect:finding-designs-trustfulengagement}



\subsubsection{Tutorials}
\hfill

\noindent
\textit{``We have grown up in this age of computers, cell phones, etc, but older adults don't (…) They don't know what it consists of, how it's going to help them, how it's not going to help them''} (C5)
\textit{``If there are some types of tutorials about the system, I am comfortable with interacting with the system''} (O5)
\textit{``I would be willing to engage interactions with the system (…) as I know little or nothing about technologies, some training to use the system might be needed''} (O2).

\subsubsection{Multimodal sensing \& Interactions}
\hfill

\noindent
Sensing:
\textit{``If a system relies only on wireless motion sensors, it might be difficult to monitor various situations and need too much confirmation by an older adult. I think the usage of camera-based sensors can complement wireless sensors (…) In case of an emergent situation, it would be beneficial to complement with images from the cameras to confirm the situation either by leveraging the silhouette of an older adult as additional information to predict the status or just showing it to the caregiver''} (O5).

Interaction:

\textit{``To avoid exceeding such a golden time of care, it is important to provide immediate care in an emergency situation. To realize this timely care, a system should provide a means of notifying an emergency signal passively or actively by an older adult. For instance, if an older adult falls with some consciousness and bleeding, but this older adult cannot move. In that case, it would be helpful if an older adult can make a sound of ‘sos’ and a system detects this emergent SOS signals to provide a necessary intervention''} (O4).
\textit{``There are going to be multiple emergency scenarios and we need a way to notify an emergency situation accordingly: one where an older adult is unconscious and requires relying on sensors and proactive intervention of a caregiver. The other where an older adult is conscious and can make some sounds or movements to notify an emergency situation''} (O5).
\textit{``Also having a wrist band (e.g. Apple watch) to collect additional signals or alert emergency situation would be useful too''} (O5).



\subsubsection{Explainable \& Personalized Interactions}
\hfill

\noindent
\textit{``I do not have any particular numerical values on how accurately a system makes a prediction. Instead, what is the most important for me to trust is how well a system can be adapted to my personal health situation and life patterns and provide personalized interactions''} (O4).

<Explainable>

\textit{``I won’t be able to trust this system much. If a system has a means of communicating to confirm the situation and elicit my confirmation to derive a personalized interaction, I would be able to trust this system more. In that sense, even if the system fails, if I can understand why it provides predictions and I can provide inputs to fix it, I can better trust it. Also, needs to make it diversified to understand different contexts''} (O4).


<Personalized Interaction>
\textit{``I think the most important issue is about personalization. it is important to have a way to customize the interaction way, period to improve the engagement with the system''} (O5)
\textit{``Depending on the status of an older adult, it is critical to provide an adequate communication medium''} (O5).
\textit{``I hope the system to be tailored to my patterns and provide a customized notification accordingly''} (O4). 
\textit{``it would be beneficial to provide an option to adjust the different interaction modalities. For instance, this system should provide a way to inform and control what notification will be given and how it will be given (…) you can opt-out monitoring, alerting, and interacting about a certain situation (…) Such an option to control the interactions with the system would be helpful to improve the user engagement to the system''} (O4).

<Adaptive Privacy Awareness>

\textit{``If a caregiver can have an option to view silhouette of an older adult, caregivers can make a better decision on whether a fall occurs or not and visit is necessary''} (O4).
\textit{``However, I think a camera sensor can be considered as a privacy invasion. I think it would be good to have an option of enabling complementary camera-based sensors in the case of detecting abnormal and emergent events (e.g. falls)''} (O5).



\subsubsection{Simple and intuitive designs}
\hfill

\noindent
\textit{``There is a fixed team but generally new people are always coming and going. So it would have to be something that didn't require a lot of learning and that was intuitive and simple''} (C5) 
\textit{``If there are some types of tutorials about the system, I am comfortable with interacting with the system. But of course, the system has to be easy to use''} (O5).


==> contents/design-opps_old2.tex <==
\section{Design Opportunities and Considerations}\label{sect:finding-designs}
In this section, we describe design opportunities and recommendations for the intelligent system for older adult care. Specifically, our findings include additional use cases and functionalities of the system but also ways to support more \red{trustworthy} user interactions with the system (Table \ref{tab:finding-designs}).


\subsection{Ways for Empowering \& {Trustworthy} Older Adult Care Technologies}\label{sect:finding-designs-trustfulengagement}
Older adults described that one contributing factor to their expected intention to engage with the system is to perceive the potential \red{benefits} that they might receive from the system (Section \ref{sect:finding-interaction}). Throughout our qualitative evaluation and design activities, caregivers and older adults discussed their perceived opportunities and limitations of an intelligent system for older adult care. In addition, they provided their critical perspectives on additional use cases and functionalities of the system (Section \ref{sect:finding-designs-usecases}) and ways to support more empowering and \red{trustworthy} user interactions with the system (Section \ref{sect:finding-designs-trustfulengagement}). This work discusses engagement with users as one of the driving forces to make human-centered, older care technologies along with other recommendations: (1) multimodal sensing \& omnipresent interactions, (2) explainability \& interactivity, (3) new benchmark datasets \& human-centered evaluations, and (4) intuitive designs \& tutorials. 

\subsubsection{Multimodal Sensing \& Omnipresent Interactions}\label{sect:finding-designs-trustfulengagement-multi}

This work discusses the need of exploring multimodal sensing and machine learning models \cite{perry2004multimodal,kumari2017increasing,ngiam2011multimodal} and omnipresent interactions for improving the system performance and experiences of older adult care technologies. Both caregivers and older adults have concerns about the performance and efficiency of the system (e.g. detecting an abnormal event) (Section \ref{sect:finding-limit-systemperf}). O5 commented that \textit{``If a system relies only on wireless motion sensors, it might be difficult to monitor various situations''} and recommended to \textit{``complement wireless motion sensors with images from cameras''}. As the usage of cameras might invade the privacy of an older adult, O5 further described to \textit{``leverage only the silhouette of an older adult from a camera or sensor data from a wrist band to predict the status or show it to a caregiver''} (O5). Thus, we recommend considering the potential of exploring multimodal data to improve the system performance on understanding fine-level daily activities. 

In addition, the exploitation of multimodality \cite{turk2014multimodal} and the investigation of omnipresent interactions would be also beneficial to improve user experience with the system. Older adults considered that dialogue responses of our system provide limited interactions during an emergency (Section \ref{sect:finding-limit-interact}). During the design activities, older adults elaborated on the necessity of a new interaction: \textit{``There are going to be multiple emergency scenarios and we need a way to notify an emergency situation accordingly: one where an older adult is unconscious and requires relying on sensors and proactive intervention of a caregiver. The other where an older adult is conscious and can make some sounds or movements to notify an emergent situation''} (O5). \textit{``If an older adult falls with some consciousness and bleeding, but cannot move. In that case, it would be helpful if an older adult can make a sound of `sos' and a system detects this to request assistance''} (O4). We suggest investigating various, omnipresent interaction methods using multimodality.

\subsubsection{Explainability \& Interactivity}\label{sect:finding-designs-trustfulengagement-xai}
Another important design opportunity and recommendation \red{for} more empowering and \red{trustworthy} user interactions are to make a system explainable and interactive \cite{holzinger2017we,gunning2019xai}. Older adults described that they \textit{``do not have any particular numerical values on how accurately a system makes a prediction. Instead, what is the most important for me to trust is how well a system can be adapted to my personal health situation and life patterns and provide personalized interactions''} (O4). When our system detects an abnormal event, our system explains an abnormal event with contextual information (e.g. the transition, frequency, duration, and time of activities) and allows older adults to share their information accordingly through interactive dialogue responses. As our system provides \textit{``a means of communicating to confirm the situation and derive a personalized interaction, I [an older adult] would be able to trust this system more''} (O4). Our study showed that such personalization can be realized in various aspects: \textit{`providing an adequate communication medium based on the status of an older adult''} (O5), \textit{``providing a way to inform and control what notification will be given and how it will be given (...) such as opt-out monitoring a certain situation''} (O4), and adaptive usage of multimodal sensor data to preserve the privacy of an older adult (Section \ref{sect:finding-designs-trustfulengagement-multi}).

\subsubsection{New Benchmark Datasets \& Human-Centered Evaluations}\label{sect:finding-designs-datasets}
Our study implies that there is a gap between the curated datasets \cite{ordonez2013activity,ordonez2015sensor,nweke2018deep} for the system implementation and evaluation and diverse realistic situations mentioned by older adults and caregivers. Our study identified the necessity of further investigation to create new benchmark datasets and design evaluation methods for older adult care technologies. As most datasets include the recording of sensor data from a single inhabitant \cite{ordonez2013activity,ordonez2015sensor,nweke2018deep} and a few sets of daily activities, it remains unclear how a machine learning model can perform other unseen situations, such as the presence of multiple inhabitants, disruptions of sensor data based on a request by an older adult, and expansion to a new activity. 

In addition, our study shed light on the possible disparities in older adult care services for people who cannot afford older adult care technologies. Instead of focusing on optimizing and evaluating older adult care technologies with the respect to their system performance, our work suggests the importance of investigating the ethical implications of adopting these older care technologies \cite{ho2020we}, how we can derive more equitable care services through technologies \cite{schwalbe2020artificial}, and human-centered evaluations of these technologies.



\subsubsection{Intuitive designs \& tutorials}
Both caregivers and older adults described the necessity of having an intelligent system with intuitive designs. Specifically, C5 mentioned that \textit{``there is a fixed team but generally new people are always coming and going. So it would have to be something that didn't require a lot of learning and that was intuitive and simple''} (C5). As older adults might not be familiar with recent technologies, \textit{``the system has to be easy to use''} (O5). It is important to iteratively engage with users and identify what they consider as intuitive designs and interactions of the system. 

Even if a system has user-centered and intuitive designs, we discuss that tutorials on a system would be beneficial to positively influence the acceptance and usage of a system. Prior work explored older adults' acceptance of mobile technology and described that the tutorial training significantly affected older adults' acceptance of mobile technologies \cite{wilkowska2009factors}. As older adults might not \textit{``know little or nothing about technologies''} (O2), we draw parallels with the prior work on older adults' acceptance of mobile technology \cite{wilkowska2009factors} and consider that \textit{``training to use the system might be needed''} (O2). 



\section{Limitations}
We worked with a group of caregivers and older adults, who have relatively diverse characteristics in age range, caregiving experience, and technology experience. Including both caregivers and older adults with diverse characteristics was helpful to have a holistic perspective of overall caregiving practices for older adults. However, we only recruited 14 participants (nine caregivers and five older adults) and did not get to recruit older adults, who have cognitive impairments due to their difficulty with participating in interviews, and older adults, who live in a center or alone. While our findings and design implications are applicable to intelligent, older adult care technologies in general, additional studies with larger groups of caregivers and older adults with diverse living conditions, and physical and cognitive conditions would provide additional perspectives on these technologies. 

In addition, we acknowledge the limitation of our qualitative evaluation study that relied on the video demonstration of our system functionalities.
Although prior design studies on care technologies showed the value of showing video demonstrations \cite{beer2012domesticated,lee2022enabling}, caregivers and older adults might provide new perspectives when they directly interact with the system. Therefore, future work is required to conduct an evaluation study with caregivers and older adults through direct interactions and how to improve multimodal sensing and interactions for more empowering and trustworthy older adult care technologies.


==> contents/discussion.tex <==



social economical


human-in-loop -> improving augmentation; reduce social isolation




We deem that human participation could help to
meet the challenges of building an efficient and
effective AAL system. Indeed, human participation
makes it possible to alleviate the sense of intrusion, to
diversify the service categories, to explore the potential
of the assistive devices, and also provides the elderly
people with chances to serve our society and keep
living actively.
Mutual assistance community, where people
mutually assist each other, is recommended as a
possible approach to bring human services into AAL





==> contents/systems-old.tex <==
\section{System Implementation}\label{sect:system}
Our main goal is to seek opinions and design ideas of caregivers and older adults on an intelligent system for older adult care. To \red{facilitate the elicitation of their opinions}, we developed an intelligent system that monitors the activities of an older adult using wireless motion sensors and machine learning and explains abnormal patterns with dialogue responses to provide an adequate intervention. The intelligent system consists of four major components: (a) monitoring module, (b) dialogue module, (c) interface of notifications and dialogue responses, and (d) database (Figure \ref{fig:flow-diagram}). In the following section, we will describe our sensor data and components of the intelligent system.


\begin{figure*}[t]
\centering
  \includegraphics[width=0.6\columnwidth]{figures/flow-diagram.png}
  %\caption{High-Level Flow Diagram}
\caption{High-level flow diagram of an intelligent system for older adult care}\label{fig:flow-diagram}
\end{figure*}
\begin{figure*}[t]
\centering 
\begin{subfigure}[t]{0.2\textwidth}
\centering
  \includegraphics[width=1.0\columnwidth]{figures/interface-notification.png}
  \caption{}
  \label{fig:system-int-noti}
\end{subfigure}\hspace{5mm}
\begin{subfigure}[t]{0.4\textwidth}
\centering
  \includegraphics[width=1.0\columnwidth]{figures/interface-dialogue-explain.png}
  \caption{}
  \label{fig:system-int-diag-explain}
\end{subfigure}%\vspace{5mm}
\begin{subfigure}[t]{0.35\textwidth}
  \centering
  \includegraphics[width=1.0\columnwidth]{figures/interface-dialogue-followup.png}
  \caption{}
  \label{fig:system-int-diag-follow}
\end{subfigure}
\caption{Interface of the System: (a) Notification about an abnormal event, (b) Dialogue responses to explain an abnormal event, and (c) Dialogue response to follow-up with an older adult.}\label{fig:system-int}
\end{figure*}

For monitoring the daily activities of an older adult, we decided to utilize wireless motion sensors instead of using a camera to preserve the privacy of an older adult (Table \ref{tab:findings-requirements}) \cite{czaja2013older}. This work assumes that wireless motion sensors have been deployed in the house of an older adult or a care center. Given sensor data based on the activities of an older adult, the monitoring module will first recognize the activity of daily livings and then detect whether a recognized activity pattern is abnormal or not. If the monitoring module detects any abnormal event, the system will send a notification to a caregiver on the web-based interface \red{(Figure \ref{fig:system-int-noti})}. As the abnormal notification does not provide sufficient information on the status of an older adult, our system can explain the contextual information of an abnormal event to a caregiver \red{(Figure \ref{fig:system-int-diag-explain})}. If this explanation is still not sufficient, a caregiver can request our system to elicit any missing information to confirm the status of an older adult. Then, the system recognizes the activities of an older adult to determine an adequate moment for the interaction (e.g. taking a rest or being idle) and prompt dialogue responses (\red{(Figure \ref{fig:system-int-diag-follow})}) to seek out the requested information from a caregiver (Table \ref{tab:findings-requirements}). All sensor readings indicate the presence in a specific area (e.g. sitting on a couch or lying in a bed) or occurrence in a particular event (e.g. cupboard open or toilet being flushed) by a single inhabitant. 

\subsection{Sensor Data and Monitoring Module}
For the development of a monitoring module, we utilized the released dataset from the work of Ord{\'o}{\~n}ez et al. \cite{ordonez2013activity} that records 21 days of activities using 12 wireless \red{motion} sensors with the labels of 11 activities of daily living.  We selected to explore this dataset to implement our system, because this dataset includes major daily activities that most caregivers leverage to understand the status of an older adult (Table \ref{tab:findings-requirements}). 

Specifically, we utilize the Hidden Markov Model (HMM) \cite{rabiner1989tutorial} that is well known to represent this problem of activity recognition \cite{ordonez2014home}. For the HMM, a hidden variable is the activity label ($y = {\vec{y_{1}}, \vec{y_{2}}, ..., \vec{y_{T}}}$) and the observation variable is the vector of sensor readings ($x = {\vec{x_{1}}, \vec{x_{2}}, ..., \vec{x_{T}}}$) for a total $T$ time slices. The joint probability of model is expressed as follows: $p(y_{1:T}, x_{1:T}) = \prod_{t=1}^T p(\vec{x_t}|\vec{y_t})p(\vec{y_t}|\vec{y_{t-1}})$.
Given fully labeled data, we learn the parameters using maximum likelihood \cite{rabiner1989tutorial}. For the evaluation of activity recognition, we apply the leave-one-day-out cross-validation and achieve 0.85 accuracy and 0.62 F1-score. 



As activity of daily livings (ADLs) are commonly utilized to assess the cognitive and physical capabilities of an older adult \cite{katz1963studies}, this work particularly focuses on developing a system that monitors ADLs. For the development of a monitoring module, we utilized the released dataset from the work of Ord{\'o}{\~n}ez et al. \cite{ordonez2013activity} that records 21 days of activities using 12 wireless sensor with the labels of 11 ADLs: \textit{``Leaving''}, \textit{``Toileting''}, \textit{``Showering''}, \textit{``Sleeping''}, \textit{``Breakfast''}, \textit{``Dinner''}, \textit{``Idle/Unlabeled''}, \textit{``Lunch''}, \textit{``Snack''}, \textit{``SpareTime/TV''}, and \textit{``Grooming''}. We selected to explore this dataset to implement our system, because this dataset includes major daily activities that most caregivers leverage to understand the status of an older adult (Table \ref{tab:findings-requirements}). 

All sensor readings indicate the presence in a specific area (e.g. sitting on a couch or lying in a bed) or occurrence in a particular event (e.g. cupboard open or toilet being flushed) by a single inhabitant. These measurements of the sensor values are discretized into time granularity $\Delta t$ = 60 seconds, which is experimented with as the best time slice from \cite{van2011human}.
Let denote a sensor event for each time slice t as $x_t^i$, where $x_t^i \in \{0, 1\}$. In a home with N binary sensor events, an observation vector is represented as $\vec{x_t} = (x_t^1, x_t^2, ..., x_t^{N-1}, x_t^{N})^T$. Our feature representation indicates when a sensor event takes place.

\subsection{Database}
We implemented a Publish-Subscribe database with MongoDB, which can not only store data, but also build a communication pipeline among the modules of our systems. For example, after the monitoring module predicts activities of daily livings and their abnormalities, the monitoring module will store the output and relevant data into the database. If any abnormal event is detected and stored in the database, the database will send the corresponding outputs of a monitoring module to the notification interface or the dialogue module to explain why an abnormal event is detected through dialogue response. In addition, when a caregiver requests to clarify the information or status of an older adult, the dialogue module will store the corresponding request to the database and prompt back to an older adult later.

\subsection{Monitoring Module}
The monitoring module of our system includes two functionalities: activity recognition and anomaly detection. In this section, we describe the implementation details of our approach for activity recognition and anomaly detection. 
%As our work focuses on receiving opinions of caregivers and older adults, 

\subsubsection{Activity Recognition}\label{sect:monitor-hmm}
\hfill

\noindent
The goal of activity recognition is to identify which activity of daily living (ADL) is occurred given time-series sensor readings. Specifically, we utilize the Hidden Markov Model (HMM) \cite{rabiner1989tutorial} that is well known to represent this problem of activity recognition \cite{ordonez2014home}. For the HMM, a hidden variable is the activity label ($y = {\vec{y_{1}}, \vec{y_{2}}, ..., \vec{y_{T}}}$) and the observation variable is the vector of sensor readings ($x = {\vec{x_{1}}, \vec{x_{2}}, ..., \vec{x_{T}}}$) for a total $T$ time slices. The joint probability of model is expressed as follows: $p(y_{1:T}, x_{1:T}) = \prod_{t=1}^T p(\vec{x_t}|\vec{y_t})p(\vec{y_t}|\vec{y_{t-1}})$.
Given fully labeled data, we learn the parameters using maximum likelihood \cite{rabiner1989tutorial}. For the evaluation of activity recognition, we apply the leave-one-day-out cross-validation and achieve 0.85 accuracy and 0.62 F1-score. 

We find that prior work explored various complex machine learning algorithms (e.g. recurrent neural network \cite{ordonez2016deep}, hybrid generative and discriminative model \cite{ordonez2013activity}) to improve the performance of activity recognition. As our work focuses on receiving opinions of caregivers and older adults about an intelligent system for older adult care, we prioritize implementing our whole system and conducting an evaluation study over exploring other algorithms to improve the performance of activity recognition. 


\subsubsection{Anomaly Detection}
\hfill

\noindent
In this section, we describe our implementation of anomaly detection that determines whether a recognized activity label is abnormal or not. For the implementation, we represent four contextual features of an activity: (1) the transition, (2) the duration, (3) frequency, and (4) starting hour of activity, which are clues for caregivers to understand abnormal events (Section \ref{sect:focusgroup-practices}).

For the transition of activity, we utilized the learned transition probability of the Hidden Markov Model (Section \ref{sect:monitor-hmm}) as the prior of the transition of an activity. We then computed the posterior to estimate the likelihood of transition of an activity label. For other contextual features of an activity (i.e. duration, frequency, starting hour), we assume that they follow Gaussian distribution and also compute the posterior to estimate their likelihood. 

For the abnormal data, we follow the prior work \cite{shin2011detection} to synthetically generate data, which utilizes the duration distribution that has been computed using the real dataset of daily activities (Section \ref{sect:system-sensors}). Specifically, we randomly draw the activity labels and the duration of a sample activity 
%at a particular time zone 
until it reaches a specified number of days. After generating the synthetic abnormal data, we merged the real dataset of daily activities with synthetic data and generated labels on each contextual feature. For labeling the contextual features of duration, frequency, and starting hours, we utilized the 90\% confidence intervals of corresponding Gaussian prior distribution to label an abnormal event \cite{shin2011detection}. For the contextual feature of the transition, we indicated the transition is abnormal if the transition probability of activity is below 0.05. 

Given this annotated dataset, we explored traditional supervised learning algorithms (e.g. decision tree, naive bayes, and support vector machine) with leave-one-day-out cross-validation to evaluate how well a system can detect abnormal events. Among various traditional supervised learning algorithms, we selected a decision tree model that leads to high performance along with the interpretability of a model prediction. Our decision trees achieved the following performances: 0.82 accuracy and 0.82 F1-score to detect abnormal transitions of activities, 0.83 accuracy and 0.79 F1-score to detect abnormal starting hours, 0.95 accuracy and 0.93 F1-score to detect abnormal duration, 0.99 accuracy and 0.99 F1-score to detect abnormal frequencies of activities.

\subsection{Dialogue Module}
The dialogue module is designed and implemented to support the interactions with both caregivers and older adults (Table \ref{tab:findings-requirements}). Specifically, our dialogue model focuses on (1) generating the explanation of a detected abnormal event and (2) eliciting additional information or confirming the status of an older adult.


\begin{figure*}[t]
\centering 
  \includegraphics[width=0.4\columnwidth]{figures/state-machine.png}
\caption{State machine to generate dialogue responses: When a caregiver or an older adult initiates the interface, the system will generate the greeting message at the \textit{``Init''} state. If a user requests to explain a detected activity or abnormal event, contextual information (e.g. time of a recognized activity, contextual features that contribute to an abnormal event) at the \textit{``Explain''} state. In addition, when a caregiver requests to elicit missing information, the system will be at the \textit{``Store Request''} state and store a corresponding request. When an older adult either takes a rest or is being idle, the system will prompt a question/request to elicit additional information at the \textit{``Prompt to Confirm''} state.}\label{fig:system-dialog-state-machine}
\end{figure*}

For generating dialogue responses, we designed and implemented the state machine (Figure \ref{fig:system-dialog-state-machine}), which hierarchically represents major interaction functions into multiple child states. The \textit{``Init''} state generates the greeting dialogue to the user after retrieving the name of the user from the database. 

The\textit{``Explain''} state and its child states provide an explanation of the detected activity event. They can either describe the general information of an event or explain contextual features of abnormal events.  The \textit{``Activity Events''} state will utilize the extracted information from activity recognition. The template of dialogue generation is specified as follows: \textit{``@user @what @where @when''}, where \textit{``@user''} is the name of a recognized user, \textit{``@what''} represents a verb representation of recognized activity, \textit{``@where''} describes a location of recognized activity, \textit{``@when''} is a time of recognized activity. A sample output response is described as follows: \textit{``Mike took a rest in the living room at 8:30''}.

The \textit{``Abnormal Events''} state will check which contextual feature is detected as abnormal and describe why that factor is detected as abnormal. The template of dialogue generation is specified as follows: \textit{``@user @what @abnormal\_feature. + @user @prediction''}. \textit{``@user''} and \textit{``@what''} are defined the same as described earlier: the name of a recognized user and a verb representation of a recognized activity. \textit{``@abnormal\_feature''} represents an adjective form of a feature of an abnormal detector: the adjective form of a duration feature is either longer or shorter, that of the frequency feature is either more or less, that of starting hour is either earlier or later. Based on the outcome of a decision tree for anomaly detection, we extract this \textit{``@abnormal\_feature''} information. \textit{``@prediction''} describes a verb representation of an activity that has the highest transition probabilities. A sample output response is described as follows: \textit{``Alice spent much more time in going out'' and ``Alice should have slept instead of going out''} (Figure \ref{fig:system-int-diag-explain}).

The\textit{``Follow-up''} state and its child states support communication between a caregiver and an older adult (Table \ref{tab:findings-requirements}). For instance, a caregiver can request our system to confirm additional information or the status of an older adult. If a caregiver requests an inquiry (e.g. \textit{``check if he/she has a dietary problem''}) for an older adult to the system, it will store this request into the database and generate dialogue response, such as \textit{``I will confirm whether he/she has a dietary problem''} at the \textit{``Store Request''} state. In addition, when the system recognizes the activity of an older adult that is appropriate to interact (e.g. after finishing $\textit{''SpareTime\/TV''}$ or after being $\textit{''Idle''}$), the system will prompt dialogue responses to elicit the request information from a caregiver (e.g. \textit{``I found you have an abnormal event of a toilet. I was wondering if you have any dietary problem?''}) at the \textit{``Prompt to Confirm''} state (Figure \ref{fig:system-int-diag-follow}). 


A user can provide dialogue responses to the system by either a chat interface (Section \ref{sect:system-int-dialog}) or voice using the Watson Cloud Speech-to-Text (STT) service. When a user provides any dialogue response, our dialogue module utilizes IBM Watson conversation service \cite{ibmconv} to recognize the intents or entities of the user's dialogue response using at least 5 similar representative words. Based on the recognized intents or entities of the user's dialogue responses, the state machine of our dialogue module will make a transition to a corresponding node and generate both an audio-output and text-output based on its specified template (Figure \ref{fig:system-int-diag-explain} and \ref{fig:system-int-diag-follow}). For generating an audio-output, we utilized the IBM Watson Cloud Text-to-Speech (TTS) service. 


\subsection{User Interface}\label{sect:system-int}
This section describes the user interface of our system (Figure \ref{fig:system-int}), which was implemented with HTML and CSS. This interface can provide a notification of an abnormal event and dialogue responses to a caregiver or an older adult.  

\subsubsection{Notification}\label{sect:system-int-noti}
\hfill

\noindent
The notification interface shows the prompt information about a detected abnormal event (Figure \ref{fig:system-int-noti}). This notification interface includes only brief information about an abnormal event (e.g. which abnormal activity is detected and when it has occurred). To highlight the detected abnormal event, we included red background color.

\subsubsection{Dialogue Responses}\label{sect:system-int-dialog}
\hfill

\noindent
The interface with dialogue responses aims to explain an abnormal event to a caregiver (Figure \ref{fig:system-int-diag-explain}) and elicit any additional information or status of an older adult (Figure \ref{fig:system-int-diag-follow}). A user can either type a dialogue response or use the voice recognition function by clicking a grey button at the bottom left of the Figure \ref{fig:system-int-diag-explain} and \ref{fig:system-int-diag-follow}.








